Small body harvest with the Antarctic Search for Transiting Exoplanets (ASTEP) project

Small Solar system bodies serve as pristine records that have been minimally altered since their formation. Their observations provide valuable information regarding the formation and evolution of our Solar system. Interstellar objects (ISOs) can also provide insight on the formation of exoplanetary systems and planetary system evolution as a whole. In this work, we present the application of our framework to search for small Solar system bodies in exoplanet transit survey data collected by the Antarctic Search for Transiting ExoPlanets (ASTEP) project. We analysed data collected during the Austral winter of 2021 by the ASTEP 400 telescope located at the Concordia Station, at Dome C, Antarctica. We identified 20 known objects from dynamical classes ranging from Inner Main-belt asteroids to one comet. Our search recovered known objects down to a magnitude of $V$ = 20.4 mag, with a retrieval rate of $\sim$80% for objects with $V \le $ 20 mag. Future work will apply the pipeline to archival ASTEP data that observed fields for periods of longer than a few hours to treat them as deep-drilling datasets and reach fainter limiting magnitudes for slow-moving objects, on the order of $V\approx $ 23-24 mag.

==> tables/target_fields_full.tex <==
\begin{table*}
\begin{center}

    \caption{\textbf{All processed target fields.}} \label{table:all_fields}

\begin{tabular}{lccccccccc}
\hline
Target name  & \begin{tabular}[c]{@{}c@{}}Ecliptic \\longitude \\(deg)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Ecliptic \\latitude \\(deg)\end{tabular} & \begin{tabular}[c]{@{}c@{}}RA \\(hms)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Dec \\(dms)\end{tabular} & Filter & \begin{tabular}[c]{@{}c@{}}Observed \\ hours\\ \end{tabular} & \begin{tabular}[c]{@{}c@{}}Detected \\ known objects \end{tabular} & \begin{tabular}[c]{@{}c@{}}Undetected \\ known objects \end{tabular} & \begin{tabular}[c]{@{}c@{}}Faintest \\ $\mathrm{V_{mag}}$ \end{tabular} \\ 

\hline

TOI-772  & 198.117 & --16.049 & 12 40 46 & --21 52 22 & $R$ & 15.3 & 14 & 11  & 20.4 \\

TOI-1955 & 43.157  & --71.902 & 04 33 40 & --51 57 22 & $R$ & 1.7 & 1 & 1 & 19.0 \\

TOI-823  & 229.541 & --24.235 & 14 34 38 & --40 44 23 & $R$ & 7.8 & 2 & 2 & 18.6 \\

TOI-283  & 187.709 & --78.424 & 07 54 17 & --65 26 29 & $R$ & 9.0 & 1 & 1 & 17.0 \\

TOI-1130 & 282.800 & --18.729 & 19 05 30 & --41 26 15 & $R$ & 7.7 & 2 & 4 & 18.8 \\

HD1397b  & 319.958 & --58.526 & 00 17 47 & --66 21 32 & $R$ & 4.4 &   &   &      \\

HD37781  & 77.569  & --73.848 & 05 38 17 & --50 38 27 & $R$ & 4.2 &   &   &       \\

TOI-1027 & 181.303 & --32.063 & 11 08 32 & --29 39 11 & $R$ & 6.8 &   &   &       \\

TOI-1041 & 177.183 & --64.697 & 09 13 36 & --55 11 52 & $R$ & 1.0 &   &   &        \\

TOI-1054 & 291.765 & --33.280 & 20 08 27 & --54 19 03 & $R$ & 2.1 &   &   &        \\

EBLM-J0608-59      &  98.847  & --82.915 & 06 08 31   & --59 32 28 & $R$ & 61.6 &   & & \\

J0600    & 90.014  & --54.448 & 06 00 00 & --31 00 27 & $R$ & 24.6 &  &   &      \\

KELT-10b & 280.811 & --24.109 & 18 58 11 & --47 00 11 & $R$ & 5.3  &  &   &      \\

NGC6208  & 257.922 & --31.024 & 16 49 28 & --53 43 41 & $R$ & 43.0 &  &   &       \\

NGC6253  & 259.423 & --29.825 & 16 59 04 & --52 42 29 & $R$ & 44.9 &  &   &       \\

TOI-1057 & 243.134 & --74.101 & 08 31 58 & --78 24 26 & $R$ & 2.8  &  &   &       \\

TOI-1064 & 289.185 & --25.84  & 19 44 00 & --47 33 41 & $R$ & 33.5 &  &   &       \\

TOI-1074 & 288.772 & --51.222 & 20 43 02 & --72 00 37 & $R$ & 21.3 &  &   &       \\

TOI-1082 & 274.299 & --75.643 & 05 33 06 & --80 48 56 & $R$ & 9.2  &  &   &       \\

TOI-1083 & 272.759 & --64.143 & 19 47 18 & --87 19 17 & $R$ & 8.6  &  &   &       \\

TOI-1105 & 268.87  & --66.851 & 09 44 15 & --89 28 17 & $R$ & 9.8  &  &   &       \\

TOI-12   & 238.50  & --42.188 & 14 35 39 & --60 10 02 & $R$ & 144.0 & &   &       \\

TOI-1214 & 272.974 & --61.165 & 19 00 11 & --84 26 53 & $R$ & 7.9  &  &   &       \\

TOI-1227 & 233.977 & --59.386 & 12 27 04 & --72 27 06 & $R$ & 6.2  &  &   &       \\

TOI-1232 & 170.251 & --77.673 & 07 46 00 & --61 52 47 & $R$ & 13.7 &  &   &       \\

TOI-14   & 76.591  & --65.793 & 05 30 14 & --42 41 52 & $R$ & 11.4 &  &   &       \\

TOI-173  & 293.773 & --70.222 & 02 13 49 & --80 34 58 & $R$ & 4.8  &  &   &       \\

TOI-174  & 358.264 & --74.961 & 03 41 50 & --62 46 01 & $R$ & 9.4  &  &   &       \\

TOI-1793 & 200.667 & --55.413 & 10 59 26 & --56 37 22 & $R$ & 5.5  &  &   &       \\

TOI-1891 & 326.51  & --36.334 & 23 02 31 & --46 05 06 & $R$ & 3.8  &  &   &       \\

TOI-190  & 5.023   & --59.089 & 02 27 06 & --50 17 04 & $R$ & 1.5  &  &   &       \\

TOI-1934&223.223&-16.233&14 20 29&-31 12 07&R&4.1&&& \\
TOI-1938&230.592&-25.26&14 37 33&-42 01 45&R&8.9&&& \\
TOI-1968&232.061&-40.237&14 08 46&-56 19 20&R&6.5&&& \\
TOI-1978&202.145&-59.005&10 44 33&-59 44 15&R&1.7&&& \\
TOI-199&51.75&-82.007&5 20 25&-59 53 44&R&9.4&&& \\
TOI-200&206.496&-68.382&9 45 35&-66 41 12&R&9.1&&& \\
TOI-2005&187.318&-45.203&10 56 07&-43 22 36&R&9.8&&& \\
TOI-201&82.654&-78.285&5 49 36&-54 54 38&R&1.4&&& \\
TOI-208&317.622&-76.116&3 33 07&-72 44 39&R&24.1&&& \\
TOI-209&326.335&-63.609&1 17 34&-66 54 09&R&42.0&&& \\
TOI-213&321.382&-71.703&2 35 32&-71 37 26&R&8.2&&& \\
TOI-215&325.121&-57.732&0 29 16&-63 47 26&R&8.2&&& \\
TOI-216&18.505&-82.482&4 55 55&-63 15 36&R&36.2&&& \\
TOI-2194&295.021&-10.394&19 56 36&-31 20 07&R&0.9&&& \\
TOI-2202&313.13&-75.346&3 24 54&-73 57 27&R&34.2&&& \\
TOI-2221&305.305&-12.823&20 45 09&-31 20 27&R&11.8&&& \\
TOI-223&331.481&-15.805&22 38 42&-25 37 54&R&6.5&&& \\
TOI-229&348.352&-34.658&0 20 57&-35 59 53&R&5.1&&& \\
TOI-2310&12.346&-76.085&4 06 05&-60 28 02&R&16.0&&& \\
TOI-2326&333.697&-32.8&23 21 57&-40 10 27&R&7.7&&& \\
TOI-2333&5.242&-72.967&3 36 53&-60 03 41&R&53.4&&& \\
TOI-2338&76.614&-57.708&5 25 22&-34 40 05&R&6.7&&& \\
TOI-2339&131.52&-76.524&7 03 02&-55 22 05&R&10.0&&& \\
TOI-2344&265.048&-52.5&17 10 51&-75 43 48&R&28.6&&& \\
TOI-2360&341.728&-72.915&3 06 38&-66 00 28&R&12.9&&& \\
TOI-2393&352.668&-62.369&2 11 46&-56 45 22&R&8.4&&& \\
TOI-240&351.028&-45.391&0 59 01&-44 09 38&R&0.7&&& \\
TOI-2416&6.452&-74.635&3 49 21&-60 47 13&R&6.2&&& \\
TOI-2419&12.478&-70.294&3 33 04&-56 35 18&R&31.2&&& \\
TOI-2463&85.994&-71.505&5 52 21&-48 05 27&R&15.5&&& \\
TOI-2525&75.548&-83.804&5 47 24&-60 31 17&R&76.1&&& \\
TOI-2526&270.068&-42.174&18 00 32&-65 36 50&R&6.6&&& \\
TOI-2531&1.338&-72.778&3 30 07&-60 52 32&R&8.9&&& \\
TOI-2536&91.649&-62.981&6 03 51&-39 32 47&R&6.9&&& \\
TOI-2540&76.591&-65.792&5 30 14&-42 41 50&R&18.3&&& \\ 
TOI-2544&154.893&-71.206&8 00 36&-54 30 32&R&13.2&&& \\
TOI-2549&143.994&-62.24&8 07 55&-44 40 00&R&43.5&&& \\
TOI-2612&70.853&-84.864&5 45 46&-61 39 36&R&7.6&&& \\
TOI-2613&326.546&-65.138&1 31 38&-67 36 35&R&12.8&&& \\
TOI-2619&327.766&-76.616&3 37 38&-70 19 50&R&4.3&&& \\
TOI-2637&172.871&-81.129&7 21 42&-64 00 51&R&17.6&&& \\
TOI-270&43.157&-71.902&4 33 39&-51 57 22&R&79.3&&& \\
TOI-282&339.493&-80.406&4 20 57&-68 06 09&R&18.8&&& \\
TOI-286&94.74&-84.09&6 03 56&-60 39 58&R&3.9&&& \\
TOI-2889&185.588&-71.452&8 48 54&-61 54 18&R&5.5&&& \\
TOI-2905&156.781&-60.273&8 43 50&-45 58 19&R&6.2&&& \\
TOI-2941&164.498&-52.755&9 25 42&-41 45 46&R&5.7&&& \\
TOI-296&332.316&-38.74&23 32 25&-45 54 34&R&35.3&&& \\
TOI-3048&219.716&-57.14&11 51 11&-65 19 00&R&8.6&&& \\
TOI-3066&188.665&-60.747&9 59 45&-56 04 40&R&6.3&&& \\
TOI-3085&202.181&-63.899&10 13 12&-62 52 31&R&8.7&&& \\
TOI-3086&188.184&-51.076&10 39 38&-48 32 16&R&8.7&&& \\
TOI-3136&250.259&-60.523&13 41 19&-79 24 35&R&4.2&&& \\
TOI-3179&202.903&-63.089&10 20 34&-62 39 03&R&8.2&&& \\
TOI-3223&222.79&-57.125&12 02 25&-66 31 45&R&7.1&&& \\
TOI-3331&271.11&-10.673&18 05 17&-34 06 25&R&8.1&&& \\
TOI-3336&275.824&-32.401&18 34 59&-55 39 48&R&9.9&&& \\
TOI-3403&138.995&-59.557&8 02 09&-41 12 19&R&6.2&&& \\
TOI-3435&124.364&-71.004&7 05 43&-49 31 13&R&4.8&&& \\
TOI-345&349.677&-33.427&0 22 47&-34 23 31&R&15.5&&& \\
TOI-3457&246.085&-64.011&12 12 50&-79 45 26&R&1.8&&& \\
TOI-346&351.97&-37.833&0 41 22&-37 20 34&R&8.8&&& \\
TOI-4181&316.725&-73.032&2 51 14&-73 09 19&R&21.0&&& \\
TOI-4188&284.574&-29.028&19 22 41&-51 25 34&R&6.7&&& \\
TOI-4262&152.248&-62.848&8 25 20&-47 02 35&R&6.4&&& \\
TOI-431&80.646&-49.947&5 33 04&-26 43 28&R&1.7&&& \\
TOI-4404&165.825&-72.041&8 14 54&-57 25 58&R&4.5&&& \\ 
TOI-4406&341.041&-56.732&1 12 11&-56 55 31&R&3.8&&& \\
TOI-451&48.139&-57.519&4 11 51&-37 56 23&R&6.3&&& \\
TOI-476&109.563&-70.403&6 38 19&-47 36 50&R&12.8&&& \\
TOI-483&97.189&-61.655&6 17 20&-38 19 23&R&6.7&&& \\
TOI-527&107.822&-59.406&6 44 45&-36 39 26&R&2.1&&& \\
TOI-533&37.998&-84.228&5 20 13&-62 38 45&R&8.9&&& \\
TOI-553&58.687&-67.172&4 53 02&-45 32 26&R&20.2&&& \\
TOI-584&162.224&-56.091&9 10 04&-43 55 30&R&3.3&&& \\
TOI-586&134.397&-56.924&7 55 39&-37 51 27&R&1.8&&& \\
TOI-588&118.961&-68.983&6 59 00&-47 01 24&R&1.0&&& \\
TOI-615&154.609&-54.681&8 53 38&-40 32 37&R&4.9&&& \\
TOI-618&126.381&-59.959&7 30 17&-39 20 22&R&7.0&&& \\
TOI-684&194.941&-63.113&10 01 44&-59 51 00&R&8.8&&& \\
TOI-687&163.526&-57.024&9 10 41&-45 05 51&R&31.1&&& \\
TOI-695&5.46&-82.913&4 52 33&-64 55 45&R&14.3&&& \\
TOI-705&233.686&-81.737&7 05 54&-72 33 31&R&16.5&&& \\
TOI-709&34.708&-72.927&4 22 37&-54 08 49&R&20.7&&& \\
TOI-712&149.709&-88.601&6 11 44&-65 49 33&R&22.0&&& \\
TOI-715&231.594&-79.387&7 35 24&-73 34 39&R&2.9&&& \\
TOI-757&202.584&-29.239&12 31 58&-35 33 17&R&6.0&&& \\
TOI-777&206.946&-42.708&12 12 28&-49 00 27&R&16.6&&& \\
TOI-783&203.867&-51.336&11 28 37&-54 47 03&R&18.9&&& \\
TOI-790&185.491&-76.012&8 13 35&-64 05 27&R&5.5&&& \\
TOI-791&209.421&-79.062&7 53 44&-69 42 06&R&35.3&&& \\
TOI-806&299.611&-77.444&4 13 40&-76 05 51&R&6.0&&& \\
TOI-809&59.62&-83.171&5 31 55&-60 28 37&R&9.1&&& \\
TOI-813&28.453&-80.537&4 50 46&-60 54 19&R&8.8&&& \\
TOI-815&180.433&-48.823&10 23 29&-43 50 06&R&4.7&&& \\
TOI-819&212.782&-38.389&12 48 45&-47 36 49&R&7.0&&& \\
TOI-835&219.341&-46.312&12 48 13&-56 53 39&R&14.0&&& \\
TOI-836&229.627&-7.088&15 00 19&-24 27 14&R&2.9&&& \\
TOI-859&123.491&-83.747&6 28 34&-61 09 01&R&39.2&&& \\
TOI-876&82.042&-47.522&5 36 26&-24 14 38&R&2.6&&& \\
TOI-903&316.435&-77.333&3 49 57&-72 47 37&R&6.2&&& \\
TOI-904&270.243&-73.429&5 57 29&-83 07 48&R&5.1&&& \\
TOI-913&259.737&-58.635&15 38 17&-80 48 13&R&12.2&&& \\
TOI-917&2.512&-70.811&3 19 15&-59 24 00&R&6.5&&& \\
TOI-929&25.104&-53.902&3 03 37&-39 55 51&R&10.7&&& \\
TOI-932&106.357&-77.68&6 23 45&-54 34 41&R&15.4&&& \\
TOI-933&82.564&-74.425&5 47 17&-51 03 59&R&24.2&&& \\
WASP-117b&5.023&-59.089&2 27 06&-50 17 04&R&2.2&&& \\
WASP-29b&339.85&-35.265&23 51 31&-39 54 24&R&0.7&&& \\
WASP-46b&302.23&-37.757&21 14 56&-55 52 18&R&5.5&&& \\

\\                                            
\end{tabular}

\end{center}

\end{table*}           
